Cryptocurrency Bubble Detection: A New Stock Market Dataset, Financial Task & Hyperbolic Models

The rapid spread of information over social media influences quantitative trading and investments. The growing popularity of speculative trading of highly volatile assets such as cryptocurrencies and meme stocks presents a fresh challenge in the financial realm. Investigating such "bubbles" - periods of sudden anomalous behavior of markets are critical in better understanding investor behavior and market dynamics. However, high volatility coupled with massive volumes of chaotic social media texts, especially for underexplored assets like cryptocoins pose a challenge to existing methods. Taking the first step towards NLP for cryptocoins, we present and publicly release CryptoBubbles, a novel multi-span identification task for bubble detection, and a dataset of more than 400 cryptocoins from 9 exchanges over five years spanning over two million tweets. Further, we develop a set of sequence-to-sequence hyperbolic models suited to this multi-span identification task based on the power-law dynamics of cryptocurrencies and user behavior on social media. We further test the effectiveness of our models under zero-shot settings on a test set of Reddit posts pertaining to 29 "meme stocks", which see an increase in trade volume due to social media hype. Through quantitative, qualitative, and zero-shot analyses on Reddit and Twitter spanning cryptocoins and meme-stocks, we show the practical applicability of CryptoBubbles and hyperbolic models.

==> ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table*}[]
    \small
    \setlength{\tabcolsep}{1.9pt}
    \centering
        \begin{tabular}{lrrrrr}
        \toprule
        \textbf{}            & \multicolumn{5}{c}{\textbf{Task}}                                                                                                                                         \\ \cmidrule(l){2-6} 
        \textbf{Model}       & \multicolumn{3}{c}{\textbf{Bubble Span}}                                                             & \multicolumn{2}{c}{\textbf{Number of Bubbles}}                     \\ \cmidrule(l){2-6} 
        \textbf{}            & \multicolumn{1}{c}{\textbf{F1$\uparrow$}} & \multicolumn{1}{c}{\textbf{MCC$\uparrow$}} & \multicolumn{1}{c}{\textbf{EM$\uparrow$}} & \multicolumn{1}{c}{\textbf{Acc (\%)$\uparrow$}} & \multicolumn{1}{c}{\textbf{F1$\uparrow$}} \\ \midrule
        EGRU & $0.48 {\scriptstyle\pm 2e-4}$  & 0.15 $\pm$ 6e-5   & 0.47 $\pm$ 3e-4   & 56.70 $\pm$ 2e-4  & 0.22 $\pm$ 1e-2                                 \\
        A-EGRU          & 0.50 $\pm$ 3e-5  & \textit{0.18 $\pm$ 1e-4}   & 0.49 $\pm$ 5e-4   & 60.48 $\pm$ 6e-5  & \textit{0.27 $\pm$ 3e-4}                                 \\
        HGRU       & \textit{0.51 $\pm$ 1e-4}  & 0.17 $\pm$ 3e-4   & \textit{0.50 $\pm$ 4e-4}   & \textit{61.03 $\pm$ 2e-4}  & 0.28 $\pm$ 3e-4                                \\
        \textbf{MBHN} & \textbf{0.53\textsuperscript{$*\dag$} $\pm$ 1e-3}  & \textbf{0.23\textsuperscript{$*\dag$} $\pm$ 4e-4}   & \textbf{0.52\textsuperscript{$*\dag$} $\pm$ 2e-3}   & \textbf{62.01\textsuperscript{$*\dag$} $\pm$ 3e-4}  & \textbf{0.29\textsuperscript{$*\dag$} $\pm$ 1e-3}                                \\ \bottomrule
    \end{tabular}
    \caption{Ablation study over the components of \textbf{MBHN} (mean of 10 independent runs). \textbf{Bold} and \textit{italics} represent \textbf{best} and \textit{second-best} results, respectively. $*$ and $\dag$ indicate statistically significant ($p<0.01$) improvement over Text- EGRU+Attention and Price-MBHN, respectively under Wilcoxon's Signed Rank Test.}
\label{tab:ablation}
\vskip -2ex
    \end{table*}
    
    

